A Study on Knowledge Distillation from Weak Teacher for Scaling Up Pre-trained Language Models

Distillation from Weak Teacher (DWT) is a method of transferring knowledge from a smaller, weaker teacher model to a larger student model to improve its performance. Previous studies have shown that DWT can be effective in the vision domain and natural language processing (NLP) pre-training stage. Specifically, DWT shows promise in practical scenarios, such as enhancing new generation or larger models using pre-trained yet older or smaller models and lacking a resource budget. However, the optimal conditions for using DWT have yet to be fully investigated in NLP pre-training. Therefore, this study examines three key factors to optimize DWT, distinct from those used in the vision domain or traditional knowledge distillation. These factors are: (i) the impact of teacher model quality on DWT effectiveness, (ii) guidelines for adjusting the weighting value for DWT loss, and (iii) the impact of parameter remapping as a student model initialization technique for DWT.

==> latex/2_related_work.tex <==


\section{Related Work}
In recent years, the use of knowledge distillation (KD)~\citep{hinton2015distilling}  has gained significant attention as a way to compress and improve the performance of large, complex language models. KD is usually used as a technique in which a smaller student model learns from a larger, pre-trained teacher model, effectively distilling the knowledge and expertise of the teacher into the student~\citep{sanh2019distilbert, wang2020minilm, wang2020minilmv2, sun-etal-2019-patient, jiao-etal-2020-tinybert}. 


In recent years, researchers have demonstrated that a variant of knowledge Distillation from Weak Teacher (DWT) can be used to improve the performance of a larger student model by transferring knowledge from a smaller or poorer teacher model~\citep{yuan2020revisiting, qin-etal-2022-knowledge}. In particular, \citet{qin-etal-2022-knowledge} have shown that DWT can be applied to pre-trained language models (PLMs) to improve performance on downstream tasks. These findings suggest that DWT has the potential to be a useful tool for optimizing the performance of large, complex models in NLP and other domains. We conduct an in-depth study and reveal the important three facts to optimize DWT on the pre-training stage of the NLP domain. 

